Henon mappings in the complex domain II: projective and inductive limits of polynomials

Let H: C^2 -> C^2 be the Henon mapping given by (x,y) --> (p(x) - ay,x). The key invariant subsets are K_+/-, the sets of points with bounded forward images, J_+/- = the boundary of K_+/-, J = the union of J_+ and J_-, and K = the union of K_+ and K_-. In this paper we identify the topological structure of these sets when p is hyperbolic and |a| is sufficiently small, ie, when H is a small perturbation of the polynomial p. The description involves projective and inductive limits of objects defined in terms of p alone.

==> GlobalMacros.tex <==
\catcode`\@=11
%
\def\singlespacing{\parskip\smallskipamount
                   \normalbaselineskip12pt
                   \normallineskip2pt
                   \normallineskiplimit1pt
                   \normalbaselines}
\def\bigsinglespacing{\parskip\medskipamount
                   \normalbaselineskip12pt
                   \normallineskip2pt
                   \normallineskiplimit1pt
                   \normalbaselines}
\def\almostdoublespacing{\parskip\smallskipamount
                   \normalbaselineskip20pt
                   \normallineskip2pt
                   \normallineskiplimit1pt
                   \normalbaselines}
\def\doublespacing{\parskip\smallskipamount
                   \normalbaselineskip24pt
                   \normallineskip2pt
                   \normallineskiplimit1pt
                   \normalbaselines}
%
\def\fulltitledpage{\pagewidth  {6.46 truein} 
                    \pageheight {8.62 truein}
                    \hcorrection{0.00 truein}
                    \vcorrection{0.00 truein}}
\def\fulluntitledpage{\pagewidth  {6.46 truein} 
                      \pageheight {9.20 truein}
                      \hcorrection{0.00 truein}
                      \vcorrection{-.44 truein}}
%
\fulltitledpage
\NoBlackBoxes
\def\parindentamount{20pt}
\parindent\parindentamount
%
\def\Aut{\qopnamewl@{Aut}{}}
\def\Id{\qopname@{Id}}
\def\id{\qopname@{id}}
\def\pr{\qopname@{pr}{}}
\def\tr{\qopnamewl@{tr}{}}
\def\ker{\qopnamewl@{ker}{}}
\def\grad{\qopnamewl@{grad}{}}
\def\diam{\qopnamewl@{diam}{}}
\def\Re{\qopnamewl@{Re}{}}
\def\Im{\qopnamewl@{Im}{}}
%
\def\set#1#2{\left\{\,#1\,\left\vert\,#2\right.\,\right\}} 
\def\altset#1#2{\left\{\,\left.#1\,\right\vert\,#2\,\right\}} 
\def\inter#1{\mathop{\kern\z@{#1}}\limits^{\circ}}
\def\A{{\Bbb A}}
\def\B{{\Bbb B}}
\def\C{{\Bbb C}}
\def\D{{\Bbb D}}
\def\E{{\Bbb E}}
\def\N{{\Bbb N}}
\def\P{{\Bbb P}}
\def\Q{{\Bbb Q}}
\def\R{{\Bbb R}}
\def\T{{\Bbb T}}
\def\Z{{\Bbb Z}}
\def\d{\partial}
\def\phi{\varphi}
\def\epsilon{\varepsilon}
\def\projlim{\varprojlim}
\def\injlim{\varinjlim}
\def\setminus{-}
\def\CmD{\C \setminus \overline D}
\def\bvec#1#2{\bmatrix#1\\#2\endbmatrix}
\def\pvec#1#2{\pmatrix#1\\#2\endpmatrix}
%
\def\cf{{\it cf.}}
\def\cp{{\it cp.}}
\def\eg{{\it e.g.}}
\def\ie{{\it i.e.}}
\def\Cf{{\it Cf.}}
\def\Cp{{\it Cp.}}
\def\Eg{{\it E.g.}}
\def\Ie{{\it I.e.}}
%
\loadbold
\loadeusm
\loadeusb
\def\script#1{{\fam\eusmfam\relax#1}}
\def\bscript#1{{\fam\eusbfam\relax#1}}
\def\citefont@{\bf}
\font\bigsmc = cmcsc10 scaled 1200
\font\bigbf  = cmbx10  scaled 1200
%
\def\today{\ifcase\month\or January\or February\or March\or
April\or May\or June\or July\or August\or September\or October\or
November\or December\fi \space\number\day, \number\year}
% 
\input psfig.tex
%
\def\setCD #1 #2 by #3 {\goodbreak\midinsert\vfill\vbox
  {\centerline{\vbox to #3{\hrule width #2 height 0pt depth 0pt\vfill
  \special{picture #1}}}}\vfill\endinsert} 
 % 
\def\settopfigure #1 #2 by #3 caption (#4) {\goodbreak\topinsert\vfill\vbox
  {\centerline{\vbox to #3{\hrule width #2 height 0pt depth 0pt\vfill
  \special{picture #1}}}\smallskip\centerline{#4}}\vfill\endinsert} 
\def\setmidfigure #1 #2 by #3 caption (#4) {\goodbreak\midinsert\vfill\vbox
  {\centerline{\vbox to #3{\hrule width #2 height 0pt depth 0pt\vfill
  \special{picture #1}}}\smallskip\centerline{#4}}\vfill\endinsert} 
\def\setpagefigure #1 #2 by #3 caption (#4) {\goodbreak\pageinsert\vfill\vbox
  {\centerline{\vbox to #3{\hrule width #2 height 0pt depth 0pt\vfill
  \special{picture #1}}}\smallskip\centerline{#4}}\vfill\endinsert} 
%
\def\settopEPSF #1 #2 by #3 caption (#4) {\goodbreak\topinsert\vfill\vbox
  {\centerline{\vbox to #3{\hrule width #2 height 0pt depth 0pt\vfill
%  \special{illustration #1}}}
   \psfig{figure=#1}}}
   \smallskip\centerline{#4}}\vfill\endinsert} 
\def\setmidEPSF #1 #2 by #3 caption (#4) {\goodbreak\midinsert\vfill\vbox
  {\centerline{\vbox to #3{\hrule width #2 height 0pt depth 0pt\vfill
%  \special{illustration #1}}}
   \psfig{figure=#1}}}
   \smallskip\centerline{#4}}\vfill\endinsert} 
\def\setPSFig #1 #2 caption (#3) {\goodbreak\midinsert\vfill\vbox
 {\centerline{\psfig{figure=#1,height=#2}}
   \smallskip\centerline{#3}}\vfill\endinsert}
\def\setpageEPSF #1 #2 by #3 caption (#4) {\goodbreak\pageinsert\vfill\vbox
  {\centerline{\vbox to #3{\hrule width #2 height 0pt depth 0pt\vfill
%  \special{illustration #1}}}
   \psfig{figure=#1}}}
  \smallskip\centerline{#4}}\vfill\endinsert} 
%
\def\settopPS #1 #2 by #3 caption (#4) {\goodbreak\topinsert\vfill\vbox
  {\centerline{\vbox to #3{\hrule width #2 height 0pt depth 0pt\vfill
%  \special{postscriptfile #1}}}
   \psfig{figure=#1}}}
  \smallskip\centerline{#4}}\vfill\endinsert} 
\def\setmidPS #1 #2 by #3 caption (#4) {\goodbreak\midinsert\vfill\vbox
  {\centerline{\vbox to #3{\hrule width #2 height 0pt depth 0pt\vfill
%  \special{postscriptfile #1}}}
   \psfig{figure=#1}}}
  \smallskip\centerline{#4}}\vfill\endinsert} 
\def\setpagePS #1 #2 by #3 caption (#4) {\goodbreak\pageinsert\vfill\vbox
  {\centerline{\vbox to #3{\hrule width #2 height 0pt depth 0pt\vfill
%  \special{postscriptfile #1}}}
   \psfig{figure=#1}}}
  \smallskip\centerline{#4}}\vfill\endinsert} 
%
\def\SetFiguresOnTop{\def\setfigure{\settopfigure} \def\setEPSF{\settopEPSF} \def\setPS{\settopPS}}
\def\SetFiguresAnywhere{\def\setfigure{\setmidfigure} \def\setEPSF{\setmidEPSF} \def\setPS{\setmidPS}}
\def\SetFiguresOnNewPage{\def\setfigure{\setpagefigure}\def\setEPSF{\setpageEPSF}\def\setPS{\setpagePS}}
%
\def\dotfil{\leaders\hbox to0.5em{\hss.\hss}\hfil}
\def\hfilll{\hskip 0pt plus 1filll}
\setbox98=\hbox{\ }
\def\QED{\setbox99=\hbox{\ \qed}
  \ifmmode\hfill\hfill\else\allowlinebreak\fi
  \hphantom{\copy99}\hskip-\wd98\kern-\wd99\hfilll\box99} 
\def\QEDL#1{\setbox99=\hbox{\ \qed~\eightpoint#1}
  \ifmmode\hfill\hfill\else\allowlinebreak\fi
  \hphantom{\copy99}\hskip-\wd98\kern-\wd99\hfilll\box99} 
%
\hyphenation {pol-y-nom-i-al}
\hyphenation {sol-e-noids}
\hyphenation {Theorem}
\hyphenation {Proposition}
\hyphenation {Lemma}
%
\newcount \chapnum
\newcount \sectionnum
\newcount \itemnum
\newcount \fignumber
\newcount \equnumber
\newcount \exercisenumber
%
\catcode`\@=\active
\endinput

